APT: Feedback-Driven Agentic Post-Training for Text-to-Image Generation

Post-training is crucial for improving text-to-image models, yet existing pipelines typically rely on manually curated training data and fixed training distributions. We introduce APT (Agentic Post-Training), a fully automated framework that adaptively post-trains a base model according to its evolving capability profile. APT coordinates three agents to construct evaluation sets from user requirements, diagnose model-specific strengths and failure modes, and generate reinforcement learning data with an adaptive prompt distribution that emphasizes underperforming capabilities. By repeatedly evaluating, diagnosing, and updating the generator, APT lets the current model's behavior shape its next training tasks, forming a feedback loop inspired by recursive self-improvement. For general-purpose settings without user-specified evaluation scenarios, we further develop an evaluation harness that enables broad and diverse evaluation set generation. Experiments across multiple base models, benchmarks, and generation architectures demonstrate that APT is model-agnostic, benchmark-agnostic, architecture-agnostic, and fully automated.

==> sections/2-related-works.tex <==
\section{Related Work}

\textbf{Post-Training for Text-to-Image Generation.}
\label{sec:related-post-train} 
Post-training has become a standard paradigm for adapting pre-trained T2I models to downstream objectives. Supervised fine-tuning (SFT) adapts a model to curated image--text pairs, with performance gains largely determined by data filtering, recaptioning, and aesthetic curation, but it remains bounded by the collected corpus and costly human curation. A complementary line directly optimizes downstream rewards following the policy-gradient view of reinforcement learning~\citep{williams1992simple, schulman2017proximal}: DDPO~\citep{black2024training} formulates denoising as a multi-step decision-making problem and optimizes diffusion models with policy gradients; Diffusion-DPO~\citep{wallace2024diffusion} adapts direct preference optimization~\citep{rafailov2023direct} to diffusion models, and SPO~\citep{liang2024step} refines it with step-aware preference signals; more recently, Flow-GRPO~\citep{flow-grpo} and follow-ups~\citep{li2025mixgrpo, liu2026policy} extend online policy-gradient training to flow matching via stochastic sampling, and DiffusionNFT~\citep{diffusionnft} performs negative-aware fine-tuning on the forward process without likelihood estimation.


\textbf{Agentic Image Generation.}
\label{sec:related-agentic} 
Recent work augments image generation and editing with agentic capabilities such as planning~\citep{agent-plan}, reasoning over implicit user intent~\citep{agent-reason}, web and image search for open-world grounding~\citep{agent-search}, and self-feedback for test-time scaling~\citep{agent-feedback-1,agent-feedback-2}, with emerging systems unifying these abilities in a single framework~\citep{agent-qwen}. 

These methods share a common design: \emph{the agent operates at inference time around a frozen generator}, improving how a fixed model is used rather than changing the model itself. As a result, intrinsic failure modes persist once the agentic scaffolding is removed, and every deployment pays the extra inference cost. 
APT instead moves the agent from the \textit{inference} loop into the \emph{post-training} loop: discover model weaknesses through evaluation and address them through training. The gains are absorbed into the model parameters and retained under standard single-pass inference, and the training distribution is re-derived from the current model at every round, making APT \emph{model-adaptive} rather than applying one fixed agentic policy to any generator. The two directions are thus complementary: prior work makes better use of a given model, while APT makes the model itself better.


